Program Repair via Direct State Manipulation

The goal of program repair is to automatically fix programs to meet a specification. We propose a new specification mechanism, direct manipulation, in which the programmer can visualize the trace of a buggy program on a failing input and convey the intended program behavior by manipulating variable values at some location. The repair problem is to find a program that, on the same input, reaches the location identified by the programmer with variable values equal to the manipulated ones. Since a single program execution under-specifies the overall program behavior, we augment our repair problem with quantitative objectives to find the program that agrees with the specification and is closest to the original one with respect to some distance. We formalize the repair problem, build a program repair tool JDial based on the Sketch synthesizer, and show the effectiveness of JDial on representative buggy benchmarks from introductory programming assignments.

==> distances.tex <==
\section{Quantitative Program Repair}
\label{sec:distances}


%\loris{
%Please make explicit that $\mathcal{R}_{LOC}(P)$ also depends on the
%  set of edits.
%}

In this section, we define program distances and  
the quantitative program repair problem.
%We define several program distances 
%to quantify syntactic or semantic changes in a program 
%due to program edits. 
%Finally, we define the quantitative program repair problem for our set-up. 
Given two programs $\Prog$, $\Progrep$ and a test set $\T$, 
a program distance\footnote{Our program distances are not necessarily {\em distance metrics}. 
In particular, some of them are not symmetric in $\Prog$ and $\Progrep$.} is a function over $\Prog$, $\Progrep$ and $\T$ 
that quantifies how {\em close} are $\Prog$ and $\Progrep$ w.r.t. $\T$. 
We classify program distances as {\em syntactic} and {\em semantic} distances. 
A syntactic program distance simply tracks the 
syntactic change between $\Prog$ and $\Progrep$, independent of the test set $\T$. Hence, a syntactic program distance is a function over $\Prog$ and $\Progrep$. 
A semantic program distance tracks the 
semantic differences between $\Prog$ and $\Progrep$ with respect to 
executions on the test set $\T$. 
In particular, a semantic program distance tracks the differences 
in the executions of $\Prog$ and $\Progrep$ on all tests $\test$ 
such that both $\Prog$ and $\Progrep$ satisfy $\test$. 
In what follows, we define several syntactic and semantic distances. 
One could easily define more sophisticated distances and we invite the reader to do so.
The following distances sufficed for our ``proof of concept'' experiments with quantitative program repair.  

\subsection{Syntactic Distances}
A syntactic distance between programs $\Prog$ and $\Progrep$ is defined 
modulo an {\em expression distance} $\expdist$. An expression distance 
tracks the syntactic difference between two expressions. In this work, 
we use two simple expression distances, defined below.

\mypar{Boolean expression distance, $\expdist_{\textsc{bool}}$,} is a 
Boolean-valued distance 
that simply tracks if two expressions are equal or not:
\begin{align*}
\expdist_{\textsc{bool}}(\expr, \exprrep) &=  
\begin{cases}
0 & \text{if } \expr = \exprrep \\
1 & \text{otherwise}.
\end{cases}
\end{align*}

\mypar{Expression-size distance, $\expdist_{\textsc{size}}$,} 
tracks the size of the repaired expression:
\begin{align*}
\expdist_{\textsc{size}}(\expr, \exprrep) &=  
\begin{cases}
0 & \text{if } \expr = \exprrep \\
size(\exprrep) & \text{otherwise}, 
\end{cases}
\end{align*}
where $size(\exprrep)$ can be defined in different ways. 
For example, $size(\exprrep)$ 
could be the total number of symbols and operators in $\exprrep$. 
In Section \ref{sec:algorithm}, we present the definition of $size(\exprrep)$ used in our implementation.
Note that $\expdist_{\textsc{size}}(\expr, \exprrep)$ is not a symmetric function. 

A syntactic program distance between programs $\Prog$ and $\Progrep$ 
is finite only if $\Prog$ and $\Progrep$ can be obtained from each 
other by applying a set of permissible program edits.
Given an expression distance $\expdist$, a syntactic program 
distance accumulates the expression distance across all expression changes between 
$\Prog$ and $\Progrep$. 
Formally:
\begin{align*}
\dsyn^{\expdist}(\Prog, \Progrep) &= 
\begin{cases}
\infty & \text{if } \forall \loc: \Progrep \not\in \Rep_\loc(\Prog) \\
\underset{\ell \in \loc: \Progrep \in \Rep_\loc(\Prog)}{\sum} \expdist(\expr_\ell, \exprrep_\ell) & \text{otherwise}.
\end{cases}
\end{align*}
Note that Prop.~\ref{prop:uniqueloc} ensures the uniqueness of $\loc$ in the second case. 
Here, $\expr_\ell, \exprrep_\ell$ denote expressions in $\ell$-labeled statements of $\Prog$, $\Progrep$, respectively. 
Thus, if $\expdist = \expdist^{\textsc{bool}}$, $\dsyn^{\expdist}(\Prog, \Progrep)$  equals 
the number of permissible program edits required to transform $\Prog$ to 
$\Progrep$. 
Similarly, if $\expdist = \expdist_{\textsc{size}}$, $\dsyn^{\expdist}(\Prog, \Progrep)$ 
equals the total size of all new expressions in $\Progrep$. 

\begin{example}\label{ex:syntactic}
Consider the programs in Figure~\ref{fig:directfixex}. 
For $\expdist = \expdist_{\textsc{bool}}$, one can see that $\dsyn^{\expdist}(\textsc{FindCBuggy},$ $\textsc{FindCBadFix})$ and 
$\dsyn^{\expdist}(\textsc{FindCBuggy},\textsc{FindCGoodFix})$ 
both equal 1, as there is exactly one permissible program edit in each case. 
For $\expdist = \expdist_{\textsc{size}}$, 
if expression size is given by the total number of symbols and operators, 
$\dsyn^{\expdist}(\textsc{FindCBuggy},\textsc{FindCBadFix})$ and 
$\dsyn^{\expdist}(\textsc{FindCBuggy},\textsc{FindCGoodFix})$ both 
equal 3. 
Neither syntactic distance can distinguish between $\textsc{FindCBadFix}$ 
and $\textsc{FindCGoodFix}$.
\end{example}

\subsection{Semantic Distances}

The semantic distance between programs $\Prog$ and $\Progrep$ 
with respect to a test set $\T$ is defined 
modulo an {\em execution distance} $\dist$. 
An execution distance 
tracks the differences between two executions. 
In this paper, we consider three types of execution distances, defined on terminating executions. 

Let $\Tcorr \subseteq \T$ consist of all tests $\test$ such that $\Prog$ and $\Progrep$ both satisfy $\test$. 
Given a test $\test$ in $\Tcorr$, 
let $\exectest(\test)$, $\exectestrep(\test)$ denote executions of $\Prog$, $\Progrep$, respectively on $\test$. 
In what follows, we fix $\exectest(\test) = \config_0, \config_1, \ldots, \config_M$ and 
$\exectestrep(\test) =$ $\configrep_0$, $\configrep_1$, $\ldots$, $\configrep_K$. Recall that a configuration 
$\config_h$ is a tuple of the form $(\ell_h, \val_h)$.

Our execution distances essentially compute the Hamming distance between two executions, using different abstractions of configurations. 
For executions of equal lengths, this distance equals the minimum number of configuration substitutions required to transform one execution into another. 
For executions of differing lengths, this distance additionally includes the difference in the execution lengths. 
All three execution distances can be defined as follows:
\begin{align*}
\dist(\exectest(\test), \exectestrep(\test)) &= 
\begin{cases}
|M - K| \, + \, \sum_{h=0}^{min(M,K)} \;  \diff(\config_h, \configrep_h) & \text{if } M, K < \infty \\
\infty & \text{otherwise}, 
\end{cases}
\end{align*}
where the definition of $\diff(\config_h, \configrep_h)$ varies for each execution distance. 

\mypar{Concrete execution distance, $\distconc$,} compares both locations and variable values
in two executions:
$\diff_{conc}(\config_h, \configrep_h) = 0$ if $\config_h = \configrep_h$ and $1$ otherwise.

\mypar{Value execution distance, $\distval$,} only compares the variable values 
in two executions:
$\diff_{val}(\config_h, \configrep_h) = 0$ if $\val_h = \valrep_h$ and $1$ otherwise.

\mypar{Location execution distance, $\distloc$,} only compares the locations
in two executions:
$\diff_{loc}(\config_h, \configrep_h) = 0$ if $\ell_h = \ellrep_h$ and $1$ otherwise.\\

A semantic program distance between programs $\Prog$, $\Progrep$ w.r.t. test set $\T$ 
is finite only if $\Prog$ and $\Progrep$ can be obtained from each 
other by applying a set of permissible program edits and $\Tcorr$ is not empty. 
Given an execution distance $\dist$ and the set $\Tcorr$, a semantic program 
distance accumulates the execution distance between executions of $\Prog$ and $\Progrep$ 
on tests in $\Tcorr$. 
Formally:
\begin{align*}
\dsem^\dist(\Prog, \Progrep, \T) &= 
\begin{cases}
\infty & \text{if } \forall \loc: \Progrep \not\in \Rep_\loc(\Prog) \text{ or } \Tcorr \text{ is empty}\\
\underset{\test \in \Tcorr}{\sum}\;  \dist(\exectest(\test), \exectestrep(\test)) & \text{otherwise.} \\
\end{cases}
\end{align*}

\begin{figure}[!t]
\setlength{\tabcolsep}{1pt}
\begin{center}
{\footnotesize
\begin{tabular}{C{3cm}|C{14mm}|C{6mm}C{6mm}C{6mm}C{6mm}C{6mm}C{6mm}C{6mm}C{6mm}C{6mm}C{6mm}}
%\hline
%\multicolumn{11}{c}{ execution} \\ \hline\hline
 & step & $0$ & $1$ & $2$ & $3$ & $4$ & $5$ & $6$ & $7$ & $8$ & $9$ \\ \hline %\hline  
 & loc & 2 & 3  & 2 & 3 & 2 & 3 & 2 & 3 & 4 & \exit \\ %\hline
%s     &  \verb-aba?gc- & \verb-aba?gc-  & \verb-aba?gc- & \verb-aba?gc- & \verb-aba?gc- & \verb-aba?gc- & \verb-aba?gc- & \verb-aba?gc- & \verb-aba?gc- & \verb-aba?gc- \\ \hline
%c     &  \verb-?- & \verb-?-  & \verb-?- & \verb-?- & \verb-?- & \verb-?- & \verb-?- & \verb-?- & \verb-?- & \verb-?-\\ \hline
%k     &  5 & 5 & 5 & 5 & 5 & 5 & 5 & 5 & 5 & 5  \\ \hline
\textsc{FindCBuggy} & j      &  $\nd$ & 0  & 0 & 1 & 1 & 2 & 2 & 3 & 3 & \exit \\ %\hline
& o     &  $\nd$ & $\nd$  & $\nd$ & $\nd$ & $\nd$ & $\nd$ & $\nd$ & $\nd$ & $\nd$ & true \\ \hline%\hline
%\multicolumn{11}{c}{\textsc{FindCBadFix} execution} \\ \hline\hline
% & & $\configrep_0$ & $\configrep_1$ & $\configrep_2$ & $\configrep_3$ & $\configrep_4$ & $\configrep_5$ & $\configrep_6$ & $\configrep_7$ & $\configrep_8$ & $\configrep_9$ \\ \hline \hline
 & loc & 2 & 3 & 4 & \exit \\ %\hline
%s     &  \verb-aba?gc- & \verb-aba?gc-  & \verb-aba?gc- & \verb-aba?gc- \\ \hline
%c     &  \verb-?- & \verb-?-  & \verb-?- & \verb-?- \\ \hline
%k     &  5 & 5 & 5 & 5  \\ \hline
\textsc{FindCBadFix} & j      &  $\nd$ & 0  & 0 & \exit \\ %\hline
& o     &  $\nd$ & $\nd$  & $\nd$ & true \\ \hline %\hline
%& \multicolumn{11}{c}{$\diff$ of configurations} \\ \hline\hline
 & $\diff_{conc}$ &  0 & 0 & 1 & 1  \\ %\hline%\hline
$\diff$ & $\diff_{val}$ &  0 & 0 & 0 & 1  \\ %\hline%\hline
& $\diff_{loc}$ &  0 & 0 & 1 & 1 %\\ %\hline%\hline
\end{tabular}
}
\end{center}
\caption{Semantic distances between executions. We do not show the 
input variables $s$, $c$, and $k$ as their values are never modified.
\label{fig:semantic}}
\end{figure}

\begin{example}\label{ex:semantic}
The executions of \textsc{FindCBuggy} and \textsc{FindCBadFix} from Figure~\ref{fig:directfixex} on $\val$ 
such that $\tinp(s)=\verb-aba?gc-, \tinp(c)=\verb-?-, \tinp(k)=5$  are shown in Fig.~\ref{fig:semantic}. 
The last 3 rows of the table show $\diff(\config_h, \configrep_h)$ for $h = 0, 1, 2, 3$.
Note that $\diff_{val}$ doesn't distinguish between $\config_2$ and $\configrep_2$ as these configurations share the same variable values. 
The difference in lengths of the given two executions is $6$. 
Thus, for these executions, $\distconc$ =  $\distloc$ = 6 + 2 = 8, and $\distval$ = 6 + 1 = 7. 

The execution of \textsc{FindCGoodFix} on the same $\val$ with $\tinp(s)=\verb-aba?gc-, \tinp(c)=\verb-?-, \tinp(k)=5$ 
is exactly the same as the execution of \textsc{FindCBuggy} shown in Fig.~\ref{fig:semantic}. Hence, 
$\distconc$ =  $\distloc$ = $\distval$ = 0 for the executions of \textsc{FindCBuggy} and \textsc{FindCGoodFix}. 
Our semantic program distances can distinguish between \textsc{FindCBadFix} and \textsc{FindCGoodFix}. 
\end{example}


%\roopsha{Prove these are distance metrics, define distances as functions ranging over $\Realsinf$}\\
%\roopsha{Illustrate using running example}

\subsection{The Quantitative Program Repair Problem}
\label{sec:qprp}
Given a program $\Prog$ and a test set $\T$ 
such that $\Prog$ does not satisfy $\T$, 
syntactic distance functions $\dsyn^1,\ldots,\dsyn^x$, 
semantic distance functions $\dsem^1,\ldots,\dsem^y$, 
and \emph{objective functions} $f_1, \ldots, f_z$ 
over $\dsyn^1,\ldots,\dsyn^x,\dsem^1,\ldots,\dsem^y$,
%$\dsyn^{\expdist_{\textsc{bool}}}$,  $\dsyn^{\expdist_{\textsc{size}}}$ and $\dsem^{\dist}$, 
the goal of quantitative program repair is to compute 
$\Progrep$ such that:
\begin{enumerate}[(1)]
\item $\Progrep$ satisfies $\T$,  
\item there exists $\loc \subseteq \Loc$ such that $\Progrep \in \Rep_\loc(\Prog)$, and  
\item 
$\Progrep = \underset{\exists \widehat{\loc} \subseteq \Loc: \widehat{\Prog}\in \Rep_{\widehat{\loc}}(\Prog)}{\arg \min} \; \underset{1\leq i\leq z}{\textsc{aggregate}} \{ f_i(\dsyn^1(\Prog, \widehat{\Prog}),\ldots,\dsem^y(\Prog,\widehat{\Prog}, \T))\}$.
\end{enumerate}
Here \textsc{aggregate} allows multiple objective functions to be combined. For example, \textsc{aggregate}
could enforce Pareto optimality.

\begin{example}
Consider the programs in Fig.~\ref{fig:directfixex}. 
In Ex.~\ref{ex:repair}, we showed that both \textsc{FindCBadFix} and \textsc{FindCGoodFix} satisfy conditions (1) and (2) 
of the quantitative program repair problem for program
\textsc{FindCBuggy} and the test set shown in Fig.~\ref{fig:directfixex}. 

In Ex.~\ref{ex:syntactic}, we showed that both 
$\dsyn^{\expdist}(\textsc{FindCBuggy},$ $\textsc{FindCBadFix})$ and 
$\dsyn^{\expdist}(\textsc{FindCBuggy},\textsc{FindCGoodFix})$ 
equal 1 for $\expdist = \expdist_{\textsc{bool}}$.
For $\expdist = \expdist_{\textsc{size}}$, 
$\dsyn^{\expdist}(\textsc{FindCBuggy},\textsc{FindCBadFix})$ and 
$\dsyn^{\expdist}(\textsc{FindCBuggy},\textsc{FindCGoodFix})$ both 
equal 3. 

The set $\Tcorr$ consists of the last two tests in the test set $\T$ in Fig.~\ref{fig:directfixex}. 
Let the test with $s=\verb-aba?gc-$ be denoted $\test_1$ and 
the test with $s=\verb-?aba-$ be denoted $\test_2$. 
Let $\exectest(\test_1)$ and $\exectest(\test_2)$ denote the executions of 
\textsc{FindCBuggy} on $\test_1$ and $\test_2$, respectively. 
Let $\exectestrep(\test_1)$, $\exectestrep(\test_2)$ and 
$\exectest''(\test_1)$, $\exectest''(\test_2)$ denote the executions of 
$\textsc{FindCBadFix}$ and $\textsc{FindCGoodFix}$ on 
$\test_1$, $\test_2$, respectively. 

We have seen in  Ex.~\ref{ex:semantic} that 
$\distconc(\exectest(\test_1), \exectestrep(\test_1)) = 8$ 
and $\distconc(\exectest(\test_1), \exectest''(\test_1)) = 0$.
It's not hard to see that 
$\distconc(\exectest(\test_2), \exectestrep(\test_2)) = 0$ 
and $\distconc(\exectest(\test_2), \exectest''(\test_2)) = 0$.
Thus, we can compute $\dsem^{\distconc}(\textsc{FindCBuggy},$ $\textsc{FindCBadFix}, T) = 8$ 
and $\dsem^{\distconc}(\textsc{FindCBuggy}, \textsc{FindCGoodFix}, T) = 0$.

If we choose $\dsyn^{\expdist_{\textsc{bool}}}$, $\dsyn^{\expdist_{\textsc{size}}}$ 
as our syntactic distances, $\dsem^{\distconc}$ as our semantic distance and 
our objective function $f$ to simply be the sum of  $\dsyn^{\expdist_{\textsc{bool}}}$, $\dsyn^{\expdist_{\textsc{size}}}$ 
and $\dsem^{\distconc}$, the value of $f$ is $4$ for \textsc{FindCGoodFix} and is $12$ for 
\textsc{FindCBadFix}. 
Hence, this instance of the quantitative program repair problem will prefer the program 
\textsc{FindCGoodFix} as a repair candidate.
\end{example}



==> encoding.tex <==
\section{MaX-SMT Encoding}
\label{sec:encoding}

\subsection{Encoding Distances}

\subsection{Encoding Program Repair}




==> iterative-figure.tex <==
\lstset{
  xleftmargin=0ex
}
\def\scalefig{0.33}
\begin{figure}[!t]
	\begin{tabular}{c;{1pt/4pt}c;{1pt/4pt}c}
		
		\begin{minipage}{\scalefig\linewidth}
			{
				\begin{lstlisting}[mathescape=true]
p = [2,1], x = 2 

int ePoly-1(int[]p,int x){
   int n = p[0];
   int i = p.Length-1;
   while(i >= 0){
     n += p[i]*pow(x,i);
     i--;
   }
$\color{gray}\rightarrow~\!$return n;
}
				\end{lstlisting}
			}
		\end{minipage}
		
		& 
		\begin{minipage}{\scalefig\linewidth}
			{
				\begin{lstlisting}[language=diff]					
int ePoly-1(int[]p,int x){
   int n = p[0]; 
   int i = p.Length-1;
   while(i >= 0){
-    n += p[i]*pow(x,i);
+    n += p[i]*pow(x,i)-1;
     i--;
   }
   return n;
}
   User disables location 
				\end{lstlisting}
			}
		\end{minipage}
		
		&
		
		\begin{minipage}{\scalefig\linewidth}
			{
				\begin{lstlisting}[language=diff]			
int ePoly-1(int[]p,int x){
   int n = p[0];
   int i = p.Length-1;
-  while(i >= 0){
+  while(i >= 1){   
     n += p[i]*pow(x,i);
     i--;
   }
   return n;
}
				\end{lstlisting}\ 
			}
		\end{minipage}
		
		
		\\
		(a) Original & (b) First repair & (c) Second repair
	\end{tabular}
	\caption{Example of direct manipulation requiring two interactions. 
	The manipulation requires  {\ttfamily n} to be 4 instead of 6 at the location
	highlighted by $\color{gray}\rightarrow$ (a). \Name generates the wrong repair (b) 
	and, after the user  disallows repairs at the modified location, 
	\Name then generates the correct  repair (c).
	}
	\label{fig:feedback}
\end{figure}

==> wrapfig-max-cegis.tex <==
\begin{wrapfigure}{r}{0.5\linewidth} 
			\begin{lstlisting}[language=diff]		
// Test: max([0,12,20])=20;
int max(int[] a){
- int max = 100;
+ int max = 0;
  for(int i=0; i<a.length; i++)
    max = Math.max(max, a[i]);
  return max;
}
			\end{lstlisting}
	\caption{Incorrect program for finding max of an array}
	\label{fig:cegismax}
\end{wrapfigure}
